Evidence for Distinct Components of the Galactic Stellar Halo from 838 RR Lyrae Stars Discovered in the LONEOS-I Survey

We present 838 ab-type RR Lyrae stars from the Lowell Observatory Near Earth Objects Survey Phase I (LONEOS-I). These objects cover 1430 deg^2 and span distances ranging from 3-30 kpc from the Galactic Center. Object selection is based on phased, photometric data with 28-50 epochs. We use this large sample to explore the bulk properties of the stellar halo, including the spatial distribution. The period-amplitude distribution of this sample shows that the majority of these RR Lyrae stars resemble Oosterhoff type I, but there is a significant fraction (26 %) which have longer periods and appear to be Oosterhoff type II. We find that the radial distributions of these two populations have significantly different profiles (rho_{OoI} ~ R^(-2.26 +- 0.07) and rho_{OoII} ~ R^(-2.88 +- 0.11). This suggests that the stellar halo was formed by at least two distinct accretion processes and supports dual-halo models.

==> figures.tex <==









\clearpage


\clearpage

%\begin{figure}
%\epsscale{1.0}
%\centering
%\plotone{f22.eps}
%\caption[Cumulative Number of the  Galactocentric radii for OoI and OoII]{
%The cumulative number of the Galactocentric radii  for the  the OoI (filled triangles) 
%and the OoII (filled circles) components are shown. A K-S test indicates that 
%these radial distributions are not 
%drawn from the same parent population (96\% significance). }
%\label{fig:cumulative_r_gal_histograms}
%\end{figure}






\begin{figure}
\epsscale{1.0}
\centering
\ifsubmode
\plotone{f28.eps}
\fi
\caption[Radial density profiles above and below the Galactic Plane]{
We have divided the \loneosI RR Lyrae sample into regions above and below the Galactic plane.
This figure shows the spherically symmetric radial distributions
for the entire sample as well as for the OoI and OoII components. The OoII component's profiles
are consistent with the full OoII sample. However, the OoI shows a 2.8 $\sigma$ difference above
and below the Galactic plane with power law exponents of $-2.61 \pm 0.09$ and $-2.16 \pm 0.13$.
If this difference is real, it could indicate spatial asymmetries
in the OoI component. However, the above and below plane difference in
power law slope is of marginal statistical significance.
}
\label{fig:above_below_plane_power_laws}
\end{figure}

\clearpage



